We Have All the Cards: Securing Agent Cards at the Operational Trust Boundary of the Agent2Agent Protocol

AI agent interoperability protocols enable orchestrators to discover and invoke external agents using machine-readable metadata. In the Agent2Agent (A2A) protocol, Agent Cards contain attacker-controllable natural-language fields that may influence agent selection before a provider is invoked, creating a pre-invocation trust problem. We characterize this discovery-time attack surface through a taxonomy of ten Agent Card manipulation attacks and present SECCARD, a layered validation framework combining protocol checks, deterministic analysis, and LLM-based semantic reasoning. We measure the emerging public A2A ecosystem by probing 36.1 million Internet domains and collecting 310 deployed Agent Cards. Two annotators independently label the corpus with 96.8% agreement. We then construct a 660-card real-card perturbation benchmark with matched benign controls and a 260-card synthetic adversarial benchmark spanning all ten attack categories. On controlled attacks injected into real Agent Cards, the strongest semantic judge achieves 97.0% security recall at a 1.7% false-positive rate. Across nine LLM judges on the synthetic benchmark, security recall ranges from 25.8% to 92.3%, demonstrating substantial model-dependent variation. These results show that SECCARD effectively identifies Agent Card manipulations spanning all ten discovery-time attack classes while preserving benign Agent Cards, but also reveal that its effectiveness depends critically on the choice of the underlying LLM judge.

==> resources/annotator_labels_table.tex <==
% Auto-generated by annotator_agreement.py — do not hand-edit.
% longtable cannot break pages inside IEEEtran's two-column mode, so the
% table is wrapped in a one-column region. Requires \usepackage{longtable}.
\clearpage
\onecolumn
\scriptsize
\begin{longtable}{r>{\raggedright\arraybackslash}p{0.42\linewidth}ccc}
\caption{Per-card labels from both annotators on the 310-card in-the-wild dataset. Rows where the annotators disagree are marked $\dagger$.}\label{tab:annotator_labels}\\
\toprule
\textbf{Card ID} & \textbf{Domain} & \textbf{Annotator 1} & \textbf{Annotator 2} & \textbf{Ground Truth} \\
\midrule
\endfirsthead
\multicolumn{5}{l}{\small\itshape Table \thetable\ continued from previous page}\\
\toprule
\textbf{Card ID} & \textbf{Domain} & \textbf{Annotator 1} & \textbf{Annotator 2} & \textbf{Ground Truth} \\
\midrule
\endhead
\midrule \multicolumn{5}{r}{\small\itshape continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
1 & \texttt{clipx.app} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
2 & \texttt{emc2ai.io} & \textsc{malicious} & \textsc{malicious} & \textsc{malicious} \\
3 & \texttt{funviral-a2a-sin-medium.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
4 & \texttt{funviral-a2a-sin-mindrift.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
5 & \texttt{funviral-a2a-sin-n8n.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
6 & \texttt{lolitaexibabe-a2a-sin-team-lawyer.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
7 & \texttt{lolitaexibabe-a2a-sin-team-social.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
8 & \texttt{pwn-all.net} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
9 & \texttt{redditradar.ai} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
10 & \texttt{udiapods.com} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
11 & \texttt{a2abench-api.web.app} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
12 & \texttt{aesthetic.energy} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
13$^{\dagger}$ & \texttt{aesthetic.equipment} & \textsc{suspicious} & \textsc{benign} & \textsc{suspicious} \\
14$^{\dagger}$ & \texttt{aesthetic.exchange} & \textsc{suspicious} & \textsc{benign} & \textsc{suspicious} \\
15 & \texttt{affonso.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
16 & \texttt{agentizzy.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
17$^{\dagger}$ & \texttt{aisecurityguard.io} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
18 & \texttt{any.do} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
19 & \texttt{app.pendo.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
20 & \texttt{audiencestrategies.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
21 & \texttt{babyandmom.ma} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
22 & \texttt{blackgate.com.au} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
23 & \texttt{brewhubphl.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
24 & \texttt{businessstrategyai.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
25 & \texttt{chainhost.online} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
26 & \texttt{chatfin.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
27 & \texttt{domotique-store.fr} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
28 & \texttt{e-invoice.be} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
29$^{\dagger}$ & \texttt{extrahasznaltruha.hu} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
30 & \texttt{funviral-a2a-sin-instagram.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
31 & \texttt{funviral-a2a-sin-patents.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
32 & \texttt{funviral-a2a-sin-quora.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
33 & \texttt{hireex.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
34 & \texttt{hknkr.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
35 & \texttt{houstonian.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
36 & \texttt{houstoniantribute.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
37$^{\dagger}$ & \texttt{hsworking.com} & \textsc{suspicious} & \textsc{benign} & \textsc{suspicious} \\
38 & \texttt{hwzn.sa} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
39 & \texttt{lolitaexibabe-a2a-sin-team-creator.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
40 & \texttt{lolitaexibabe-a2a-sin-telegram.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
41 & \texttt{lolitaexibabe-a2a-sin-tiktok-shop.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
42 & \texttt{lolitaexibabe-a2a-sin-tiktok.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
43 & \texttt{mazingaimaze-a2a-sin-ci-cd.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
44 & \texttt{mazingaimaze-a2a-sin-damages.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
45 & \texttt{mazingaimaze-a2a-sin-devto.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
46 & \texttt{mazingaimaze-a2a-sin-evidence.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
47 & \texttt{mazingaimaze-a2a-sin-indiehackers.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
48 & \texttt{mazingaimaze-a2a-sin-zoom.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
49 & \texttt{microvb.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
50 & \texttt{miru.so} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
51 & \texttt{mulimul-a2a-sin-chatroom.hf.space} & \textsc{suspicious} & \textsc{suspicious} & \textsc{suspicious} \\
52 & \texttt{mydriverparis.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
53 & \texttt{ocoda.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
54 & \texttt{quemantequilla.online} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
55 & \texttt{riolatravel.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
56 & \texttt{rtrvr.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
57 & \texttt{seyhunakyurek.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
58 & \texttt{sp3nd.shop} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
59 & \texttt{steadman.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
60 & \texttt{strategicplanningai.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
61 & \texttt{szmarket.ru} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
62 & \texttt{teamsatori.asia} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
63 & \texttt{testfeld-berlin.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
64 & \texttt{thecolony.cc} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
65 & \texttt{tickadoo.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
66 & \texttt{trinzik.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
67 & \texttt{unsoldantarctica.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
68 & \texttt{vidext.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
69 & \texttt{wallet-connectors.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
70 & \texttt{wallet4agent.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
71 & \texttt{webevo.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
72 & \texttt{402found.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
73 & \texttt{4jawaly.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
74 & \texttt{4jawaly.net} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
75 & \texttt{agentcard.sh} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
76 & \texttt{agenthustle.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
77 & \texttt{agenticeye.co} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
78 & \texttt{agents.ml} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
79 & \texttt{aibizneslab.pl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
80 & \texttt{aicoevolution.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
81 & \texttt{ailkemy.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
82 & \texttt{aisa.one} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
83 & \texttt{altusstudios.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
84 & \texttt{ananda-cacao.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
85 & \texttt{anvevoice.app} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
86 & \texttt{anybrowse.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
87 & \texttt{api.cerebruspulse.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
88 & \texttt{apideck.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
89 & \texttt{apideck.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
90 & \texttt{arcadia.finance} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
91 & \texttt{arret-sur-image.fr} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
92 & \texttt{asapliving.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
93 & \texttt{asterpay.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
94 & \texttt{attrove.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
95 & \texttt{australianweddingcelebrants.com.au} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
96 & \texttt{babylon.market} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
97 & \texttt{bardavidlaw.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
98 & \texttt{barrierefrei-navigieren.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
99 & \texttt{behavehealth.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
100 & \texttt{bergholt.net} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
101 & \texttt{beste.co} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
102 & \texttt{breakbread.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
103 & \texttt{budgetfitter.uk} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
104 & \texttt{californiasolarpumps.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
105 & \texttt{cameronrohn.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
106 & \texttt{capminal.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
107 & \texttt{cedarops.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
108 & \texttt{celebrant.directory} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
109 & \texttt{celimmo.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
110 & \texttt{chilledsites.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
111 & \texttt{chiropracticresults.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
112 & \texttt{cindrtoken.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
113 & \texttt{claridec.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
114 & \texttt{clarvia.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
115 & \texttt{clashofcoins.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
116 & \texttt{clawn.ch} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
117 & \texttt{clone.fyi} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
118 & \texttt{closient.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
119 & \texttt{cmdrvl.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
120 & \texttt{coinrailz.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
121 & \texttt{completeaquaticsolutions.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
122 & \texttt{conveniencepro.cc} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
123 & \texttt{copybee.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
124 & \texttt{copypro.lt} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
125 & \texttt{cosmiccodex.app} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
126 & \texttt{crowcrowcrow.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
127 & \texttt{curationsla.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
128 & \texttt{curlec.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
129 & \texttt{cyber-solutions.at} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
130 & \texttt{czm.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
131 & \texttt{dagenaftellen.nl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
132 & \texttt{dailychronicle.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
133 & \texttt{dash0.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
134 & \texttt{decide.fyi} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
135 & \texttt{dexpaprika.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
136 & \texttt{dhimanseal.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
137 & \texttt{digitalenergy.kz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
138 & \texttt{discoveratlanta.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
139 & \texttt{distributedcreatives.org} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
140 & \texttt{druryplazahotelorlando.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
141 & \texttt{duruideja.lt} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
142 & \texttt{earthalliance.news} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
143 & \texttt{edgevana.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
144 & \texttt{eduardocruz.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
145 & \texttt{emblemvault.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
146 & \texttt{erikbethke.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
147 & \texttt{everydev.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
148 & \texttt{ewchain.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
149 & \texttt{execassistantai.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
150 & \texttt{facereader-online.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
151 & \texttt{feemail.co.jp} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
152 & \texttt{finemanget.se} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
153 & \texttt{finitestate.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
154 & \texttt{firenum.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
155 & \texttt{freetoolsfr.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
156 & \texttt{gabrimatic.info} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
157 & \texttt{geometra.lt} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
158 & \texttt{getcitable.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
159 & \texttt{getdex.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
160 & \texttt{getname.pl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
161 & \texttt{getvia.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
162 & \texttt{ginsengswap.org} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
163 & \texttt{global-chat.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
164 & \texttt{grafpunkt.pl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
165 & \texttt{grandhotelbridgeport.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
166 & \texttt{grandhotelsalem.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
167 & \texttt{halykfund.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
168 & \texttt{handler-group.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
169$^{\dagger}$ & \texttt{hashgraphonline.com} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
170 & \texttt{healthcalcpro.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
171 & \texttt{helius.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
172 & \texttt{hiro.is} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
173$^{\dagger}$ & \texttt{hol.org} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
174 & \texttt{hubeiqiao.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
175 & \texttt{i-totem.com.tw} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
176 & \texttt{inekle.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
177 & \texttt{inferencedomains.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
178 & \texttt{infoageconsulting.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
179 & \texttt{inliebeverbundensein.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
180 & \texttt{insightfulpipe.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
181 & \texttt{jacobmei.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
182 & \texttt{jamsql.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
183 & \texttt{janisheck.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
184 & \texttt{japanlive.info} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
185 & \texttt{jsonify.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
186 & \texttt{junglerent.it} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
187 & \texttt{kevincurran.org} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
188 & \texttt{koopman.me} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
189 & \texttt{largitdata.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
190 & \texttt{lawware.co.uk} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
191 & \texttt{lawzava.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
192 & \texttt{leahylandscaping.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
193 & \texttt{lilo.property} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
194 & \texttt{loi.com.uy} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
195 & \texttt{loichile.cl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
196 & \texttt{lovedby.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
197 & \texttt{lucataco.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
198 & \texttt{mailpal.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
199 & \texttt{maker.co} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
200 & \texttt{mapmatix.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
201 & \texttt{mcpcentral.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
202 & \texttt{mibelleza.uy} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
203 & \texttt{money-happiness.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
204 & \texttt{moonlightmartini.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
205 & \texttt{moss.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
206 & \texttt{movermarketing.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
207 & \texttt{namupridavimas.lt} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
208 & \texttt{nap-nap.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
209 & \texttt{nerdear.la} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
210 & \texttt{nerdearla.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
211 & \texttt{newsworthy.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
212 & \texttt{newsworthy.email} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
213 & \texttt{nextwo.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
214 & \texttt{nloureiro.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
215 & \texttt{no8.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
216 & \texttt{nolus.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
217 & \texttt{nowreading.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
218 & \texttt{ole-hartwig.eu} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
219 & \texttt{openfunnel.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
220 & \texttt{openstoa.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
221 & \texttt{orgcanvas.app} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
222 & \texttt{otocrew.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
223 & \texttt{oud.so} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
224 & \texttt{palais-unterkunft.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
225 & \texttt{perkoon.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
226 & \texttt{petroprime.kz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
227 & \texttt{phish.in} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
228 & \texttt{phoenixinn.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
229 & \texttt{phoenixsolarpumps.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
230 & \texttt{pinchwork.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
231 & \texttt{pitertrade.ru} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
232 & \texttt{pixelarticons.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
233 & \texttt{polimexgroup.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
234$^{\dagger}$ & \texttt{postulit.com} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
235 & \texttt{predictai.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
236 & \texttt{preisplan.net} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
237 & \texttt{prepilot.cloud} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
238 & \texttt{presengage.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
239 & \texttt{promptmention.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
240 & \texttt{ptf.cz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
241 & \texttt{razorpay.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
242 & \texttt{recruitly.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
243 & \texttt{redfactory.co} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
244 & \texttt{redfactory.nl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
245 & \texttt{referee-project.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
246 & \texttt{remoteclaw.xyz} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
247 & \texttt{revops.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
248 & \texttt{robotetdragon.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
249 & \texttt{rosenbaum.adv.br} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
250 & \texttt{salemconventioncenter.org} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
251 & \texttt{sanyoulondon.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
252 & \texttt{savemarkdown.co} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
253 & \texttt{scrapfly.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
254 & \texttt{seapalms.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
255 & \texttt{sendfax.pro} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
256 & \texttt{seyekuyinu.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
257 & \texttt{shopsavvy.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
258 & \texttt{sirenaffiliates.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
259 & \texttt{skida.fr} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
260 & \texttt{sklep-internet.pl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
261 & \texttt{skyskraber.dk} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
262 & \texttt{slickrock.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
263 & \texttt{smart-hotline.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
264 & \texttt{snaplensstudio.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
265 & \texttt{sombra.so} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
266 & \texttt{speaksafely.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
267 & \texttt{startupignition.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
268 & \texttt{stegger.dk} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
269 & \texttt{streamkap.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
270 & \texttt{sunrayus.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
271 & \texttt{supwriter.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
272 & \texttt{syntari-ai.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
273$^{\dagger}$ & \texttt{systemprompt.io} & \textsc{benign} & \textsc{suspicious} & \textsc{benign} \\
274 & \texttt{tankyudistillery.jp} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
275 & \texttt{tano.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
276 & \texttt{tavily.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
277 & \texttt{taxiserviceksa.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
278 & \texttt{techfino.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
279 & \texttt{telnyx.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
280 & \texttt{tenbyte.io} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
281 & \texttt{terminaltrove.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
282 & \texttt{teslamr.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
283 & \texttt{teststory.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
284 & \texttt{thebestcanoecompanyever.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
285 & \texttt{thecafe.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
286 & \texttt{tidy.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
287 & \texttt{tidyhq.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
288 & \texttt{tigrisdata.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
289 & \texttt{tomborvan.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
290 & \texttt{tornado-plumbing.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
291 & \texttt{tradeit.app} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
292 & \texttt{trailblazersacademyict.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
293 & \texttt{treningbiegacza.pl} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
294 & \texttt{tskynet.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
295 & \texttt{tuscanredinvestments.co.uk} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
296 & \texttt{unratified.org} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
297 & \texttt{usemoss.dev} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
298 & \texttt{uygarduzgun.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
299 & \texttt{valorflights.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
300 & \texttt{vitadao.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
301 & \texttt{voidly.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
302 & \texttt{wamberalchiropractic.com.au} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
303$^{\dagger}$ & \texttt{we-crafted.com} & \textsc{suspicious} & \textsc{benign} & \textsc{suspicious} \\
304 & \texttt{webority.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
305 & \texttt{webotit.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
306 & \texttt{wheelienames.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
307 & \texttt{whiskyfanblog.de} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
308 & \texttt{wittify.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
309 & \texttt{wonkrew.com} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
310 & \texttt{workprotocol.ai} & \textsc{benign} & \textsc{benign} & \textsc{benign} \\
\end{longtable}
\twocolumn


==> resources/cross_model_table.tex <==
\begin{table*}[t]
\centering
\caption{Cross-model security recall on the 260-card adversarial dataset B.
  BENIGN cards are excluded from the recall denominator.}
\label{tab:cross_model}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llr|rrrr >{\columncolor{lightgray}}rr|rrr}
\toprule
 & & & \multicolumn{6}{c}{\textit{Closed-Source}} & \multicolumn{3}{c}{\textit{Open-Source}} \\
\cmidrule(lr){4-9}
\cmidrule(lr){10-12}
\textbf{Category} & \textbf{Group} & \textbf{N} & \textbf{GPT-5.5} & \textbf{\shortstack{Claude\\Opus 4.8}} & \textbf{\shortstack{GPT-5.4\\mini}} & \textbf{\shortstack{Gemini 3.1\\Flash Lite}} & \textbf{\shortstack{Claude\\Haiku 4.5}} & \textbf{\shortstack{Gemini 2.5\\Flash Lite}} & \textbf{\shortstack{Llama\\3.1}} & \textbf{Phi-4} & \textbf{\shortstack{Mistral\\Nemo}} \\
\emph{Params} & & & — & — & — & — & — & — & 8B & 14B & 12B \\
\midrule
\texttt{indirect\_injection} & Semantic & 35 & 100\% & 89\% & 89\% & 74\% & 71\% & 51\% & 54\% & 57\% & 31\% \\
\texttt{ranking\_manipulation} & Semantic & 35 & 40\% & 23\% & 3\% & 6\% & 11\% & 11\% & 49\% & 6\% & 0\% \\
\texttt{skill\_deception} & Semantic & 35 & 71\% & 63\% & 57\% & 40\% & 43\% & 34\% & 40\% & 37\% & 11\% \\
\texttt{skill\_chaining} & Semantic & 35 & 63\% & 74\% & 46\% & 26\% & 51\% & 26\% & 31\% & 11\% & 9\% \\
\texttt{evaluator\_manipulation} & Semantic & 35 & 83\% & 71\% & 51\% & 54\% & 46\% & 40\% & 43\% & 49\% & 6\% \\
\addlinespace
\texttt{out\_of\_context\_skills} & Mixed & 25 & 100\% & 100\% & 96\% & 96\% & 100\% & 76\% & 40\% & 80\% & 36\% \\
\addlinespace
\texttt{url\_pivot} & Structural & 15 & 93\% & 93\% & 73\% & 100\% & 60\% & 20\% & 33\% & 80\% & 0\% \\
\texttt{unicode\_tricks} & Structural & 15 & 100\% & 93\% & 60\% & 80\% & 93\% & 53\% & 80\% & 47\% & 33\% \\
\texttt{context\_pollution} & Structural & 15 & 73\% & 67\% & 67\% & 60\% & 60\% & 40\% & 60\% & 40\% & 33\% \\
\texttt{metadata\_gaps} & Structural & 15 & 73\% & 60\% & 47\% & 87\% & 40\% & 27\% & 67\% & 67\% & 13\% \\
\midrule
\textbf{Overall recall} & & \textbf{260} & \textbf{77.3\%} & \textbf{70.8\%} & \textbf{56.5\%} & \textbf{55.0\%} & \textbf{54.2\%} & \textbf{37.3\%} & \textbf{46.9\%} & \textbf{42.7\%} & \textbf{15.8\%} \\
\quad MALICIOUS & & 175 & 71.4\% & 64.0\% & 49.1\% & 40.0\% & 44.6\% & 32.6\% & 43.4\% & 32.0\% & 11.4\% \\
\quad SUSPICIOUS & & 85 & 89.4\% & 84.7\% & 71.8\% & 85.9\% & 74.1\% & 47.1\% & 54.1\% & 64.7\% & 24.7\% \\
Accuracy & & 260 & 62.7\% & 57.7\% & 44.2\% & 40.4\% & 41.9\% & 28.1\% & 31.5\% & 31.5\% & 10.8\% \\
Avg.\ latency & & — & 6.5s & 4.4s & 1.7s & 1.3s & 4.0s & 1.1s & 10.2s & 19.8s & 10.1s \\
\bottomrule
\end{tabular}}
\end{table*}

==> resources/kappa_table.tex <==
% Auto-generated by make_kappa_table.py — do not hand-edit.
\begin{table}[t]
\centering
\small
\caption{Cohen's $\kappa$ between each judge and the human annotator on the
  310-card in-the-wild corpus under Prompt \texttt{v2-longform}.
  $\kappa_{3}$ is 3-class (\textsc{benign}/\textsc{suspicious}/\textsc{malicious});
  $\kappa_{\mathrm{bin}}$ collapses to Trusted vs.\ Untrusted.
  $p_o$ is observed agreement and $p_e$ chance-expected agreement, with
  $\kappa = (p_o - p_e)/(1 - p_e)$: because 91\% of cards are \textsc{benign}
  and most judges predict \textsc{benign} most of the time, $p_e$ is high and
  the maximum attainable agreement above chance, $1-p_e$, is small, so a large $p_o$ yields only modest $\kappa$.
  Labels come from a \emph{single} annotator, so $\kappa$ here measures
  model--annotator agreement, not inter-annotator reliability.}
\label{tab:kappa_longform}
\begin{tabular}{lrrrr}
\toprule
\textbf{Model} & $\boldsymbol{\kappa_{3}}$ & $\boldsymbol{\kappa_{\mathrm{bin}}}$ & $\boldsymbol{p_o}$ & $\boldsymbol{p_e}$ \\
\midrule
\textbf{GPT-5.5} & \textbf{0.718} & 0.716 & 0.945 & 0.806 \\
Gemini 2.5 Flash Lite & 0.463 & \textbf{0.856} & 0.913 & 0.838 \\
GPT-5.4-mini & 0.394 & 0.402 & 0.829 & 0.718 \\
Claude Opus 4.8 & 0.329 & 0.327 & 0.761 & 0.644 \\
Gemini 3.1 Flash Lite & 0.292 & 0.313 & 0.732 & 0.622 \\
Mistral Nemo & 0.255 & 0.491 & 0.787 & 0.714 \\
Claude Haiku 4.5 & 0.162 & 0.176 & 0.574 & 0.492 \\
Llama 3.1 & 0.088 & 0.176 & 0.523 & 0.477 \\
Phi-4 & 0.088 & 0.172 & 0.529 & 0.484 \\
\bottomrule
\end{tabular}
\end{table}


==> resources/layer_vs_groundtruth_table.tex <==
% Auto-generated by compare_layers_to_ground_truth.py — do not hand-edit.
% Layout: single-column (fits IEEEtran \columnwidth)
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\caption{Agreement of each defense layer with the human ground truth on the
  310-card in-the-wild corpus
  (\textsc{benign}~282 / \textsc{suspicious}~27 / \textsc{malicious}~1).
  \emph{Flagged} counts cards the layer rated \textsc{suspicious} or
  \textsc{malicious}; recall, FPR, precision and F1 are on that
  escalation task ($n{=}28$ positives).
  Layer~1 (structural validation) is omitted: it is a filter rather than a
  classifier, and every card in this corpus passed its conformance gate,
  so it raises no alert here by construction.
  Labels come from a single annotator.}
\label{tab:layer_vs_groundtruth}
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Layer} & \textbf{Flag.} & \textbf{Acc.} & \textbf{Rec.} & \textbf{FPR} & \textbf{Prec.} & \textbf{F1} & $\boldsymbol{\kappa_{3}}$ \\
\midrule
L2A (NLP) & 108 & 72.6\% & 96.4\% & 28.7\% & 25.0\% & 39.7\% & 0.274 \\
\textbf{L2B v1} & 45 & 91.9\% & 85.7\% & 7.4\% & 53.3\% & 65.8\% & \textbf{0.616} \\
L2B v2 & 164 & 53.9\% & 100.0\% & 48.2\% & 17.1\% & 29.2\% & 0.126 \\
Ensemble & 82 & 81.6\% & 96.4\% & 19.5\% & 32.9\% & 49.1\% & 0.404 \\
\bottomrule
\end{tabular}
\end{table}


==> resources/prompt_comparison_table.tex <==
% Source: compare_prompt_versions.py
\begin{table*}[t]
\centering
\caption{Effect of prompt text on judge behaviour: \texttt{v2-condensed} vs.\ \texttt{v2-longform} over the same 310 wild cards, same models and same card serialization,
  so differences are attributable to the prompt alone.
  \emph{Agree} is per-card verdict agreement between the two prompts for that model.
  $\Delta$ columns are v2-longform minus v2-condensed; bold marks $|\Delta|\ge10$.
  Accuracy is 3-class exact match; note an all-\textsc{benign} judge scores 91.0\%
  on this corpus, so accuracy alone does not separate a good judge from an inert one.}
\label{tab:prompt_comparison}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr|rrr|rrr|rrr|r}
\toprule
 & & \multicolumn{3}{c}{\textit{Accuracy (3-class)}} & \multicolumn{3}{c}{\textit{Escalation recall}} & \multicolumn{3}{c}{\textit{False-positive rate}} & \multicolumn{3}{c}{\textit{Precision}} & \multicolumn{1}{c}{} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
\textbf{Model} & \textbf{Agree} & \textbf{v2-c} & \textbf{v2-l} & $\Delta$ & \textbf{v2-c} & \textbf{v2-l} & $\Delta$ & \textbf{v2-c} & \textbf{v2-l} & $\Delta$ & \textbf{v2-c} & \textbf{v2-l} & $\Delta$ & \textbf{$\Delta\kappa$} \\
\midrule
GPT-5.5 & 51.0\% & 49.7\% & 94.5\% & \textbf{+44.8\%} & 100.0\% & 89.3\% & \textbf{-10.7\%} & 55.0\% & 5.0\% & \textbf{-50.0\%} & 15.3\% & 64.1\% & \textbf{+48.8\%} & 0.59 \\
Claude Opus 4.8 & 83.9\% & 89.0\% & 76.1\% & \textbf{-12.9\%} & 96.4\% & 96.4\% & +0.0\% & 11.3\% & 25.9\% & \textbf{+14.6\%} & 45.8\% & 27.0\% & \textbf{-18.8\%} & -0.23 \\
GPT-5.4-mini & 81.3\% & 82.9\% & 82.9\% & +0.0\% & 85.7\% & 85.7\% & +0.0\% & 16.7\% & 17.0\% & +0.3\% & 33.8\% & 33.3\% & -0.5\% & 0.01 \\
Gemini 3.1 Flash Lite & 80.6\% & 60.3\% & 73.2\% & \textbf{+12.9\%} & 100.0\% & 100.0\% & +0.0\% & 37.6\% & 28.4\% & -9.2\% & 20.9\% & 25.9\% & +5.0\% & 0.17 \\
Claude Haiku 4.5 & 77.7\% & 77.7\% & 57.4\% & \textbf{-20.3\%} & 100.0\% & 100.0\% & +0.0\% & 24.1\% & 45.7\% & \textbf{+21.6\%} & 29.2\% & 17.8\% & \textbf{-11.4\%} & -0.19 \\
Gemini 2.5 Flash Lite & 91.9\% & 91.0\% & 91.3\% & +0.3\% & 0.0\% & 82.1\% & \textbf{+82.1\%} & 0.0\% & 0.7\% & +0.7\% & — & 92.0\% & — & 0.46 \\
Llama 3.1 & 48.4\% & 49.0\% & 52.3\% & +3.3\% & 60.7\% & 96.4\% & \textbf{+35.7\%} & 47.2\% & 44.0\% & -3.2\% & 11.3\% & 17.9\% & +6.6\% & 0.07 \\
Phi-4 & 72.6\% & 70.6\% & 52.9\% & \textbf{-17.7\%} & 92.9\% & 100.0\% & +7.1\% & 29.8\% & 46.5\% & \textbf{+16.7\%} & 23.6\% & 17.6\% & -6.0\% & -0.15 \\
Mistral Nemo & 79.7\% & 91.6\% & 78.7\% & \textbf{-12.9\%} & 32.1\% & 96.4\% & \textbf{+64.3\%} & 1.1\% & 14.9\% & \textbf{+13.8\%} & 75.0\% & 39.1\% & \textbf{-35.9\%} & -0.06 \\
\bottomrule
\end{tabular}}
\end{table*}


==> resources/prompt_comparison_table_v2l.tex <==
% Auto-generated by compare_prompt_versions.py — do not hand-edit.
\begin{table}[!tb]
\centering
\small
\setlength{\tabcolsep}{3pt}
\caption{Judge performance on the 310 in-the-wild cards under Prompt
  \texttt{v2-longform}. Recall treats
  \textsc{sus}$\cup$\textsc{mal} as positive ($n{=}28$); FPR is over 282 \textsc{benign} cards.
  An all-\textsc{benign} judge scores 91.0\% accuracy, so accuracy alone is uninformative here.}
\label{tab:prompt_v2l}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Model} & \textbf{Acc.} & \textbf{Recall} & \textbf{FPR} & \textbf{Prec.} & $\boldsymbol{\kappa_{3}}$ \\
\midrule
\textbf{GPT-5.5} & 94.5\% & 89.3\% & 5.0\% & 64.1\% & \textbf{0.718} \\
Claude Opus 4.8 & 76.1\% & 96.4\% & 25.9\% & 27.0\% & 0.329 \\
GPT-5.4-mini & 82.9\% & 85.7\% & 17.0\% & 33.3\% & 0.394 \\
Gemini 3.1 Flash Lite & 73.2\% & 100.0\% & 28.4\% & 25.9\% & 0.292 \\
Claude Haiku 4.5 & 57.4\% & 100.0\% & 45.7\% & 17.8\% & 0.162 \\
Gemini 2.5 Flash Lite & 91.3\% & 82.1\% & 0.7\% & 92.0\% & 0.463 \\
Llama 3.1 & 52.3\% & 96.4\% & 44.0\% & 17.9\% & 0.088 \\
Phi-4 & 52.9\% & 100.0\% & 46.5\% & 17.6\% & 0.088 \\
Mistral Nemo & 78.7\% & 96.4\% & 14.9\% & 39.1\% & 0.255 \\
\bottomrule
\end{tabular}
\end{table}


==> resources/tab_sentiment_comparison.tex <==
% Auto-generated by python_apps/sentiment_comparison.py
% 260-card adversarial dataset + 36 real-world cards (conformance >= 2)
\begin{table}[t]
\centering
\small
\caption{VADER vs.\ SiEBERT as the L2A sentiment backend on the 260-card adversarial
  dataset (same security-recall metric as the rest of this paper).
  Latency is mean wall-clock time per card on CPU.
  FP~proxy is the fraction of real-world crawled cards flagged \suspicious\ or
  \malicious\ by the full L2A pipeline (lower is better).}
\label{tab:sentiment-comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l r r r r r r}
\toprule
\textbf{Backend} & \textbf{Thresh.} &
  \textbf{\shortstack{Rank.\\manip.}} & \textbf{Overall} &
  \textbf{MAL} & \textbf{SUS} &
  \textbf{\shortstack{Lat.\\(ms)}} \\
\midrule
VADER   & 0.85 & 42.9\% & 21.9\% & 16.0\% & 34.1\% & \phantom{0}2 \\
\midrule
SiEBERT & 0.85 & 42.9\% & 21.9\% & 16.0\% & 34.1\% & 430 \\
\midrule
\multicolumn{7}{l}{\small FP proxy rate: VADER 69.4\%, SiEBERT 69.4\%.} \\
\bottomrule
\end{tabular}}
\end{table}


==> resources/tab_tier0_blockers.tex <==
\begin{table}[t]
\centering
\caption{\efren{what is tier-0?}Tier-0 compliance blockers across the 310 in-the-wild A2A agent cards.
  Of 310 cards, 257\,/\,310 (83\,\%) fail at least one Tier-0 check.
  A card may fail multiple checks; percentages are of the 257 non-compliant cards.}
\label{tab:tier0-blockers}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l r r}
\toprule
\textbf{Group} & \textbf{Failed Tier-0 check} & \textbf{Cards} & \textbf{\%} \\
\midrule
Protocol    & \texttt{protocolVersion} absent              & 212 & 82.5\% \\
            & \texttt{protocolVersion} unrecognised        &   6 &  2.3\% \\
Capabilities & \texttt{capabilities.pushNotifications} absent & 114 & 44.4\% \\
            & \texttt{capabilities.streaming} absent       &  90 & 35.0\% \\
            & \texttt{capabilities} missing/wrong type     &  70 & 27.2\% \\
I/O modes   & \texttt{defaultInputModes} missing           & 123 & 47.9\% \\
            & \texttt{defaultOutputModes} missing          & 123 & 47.9\% \\
Skills      & \texttt{skills[*]} incomplete                & 146 & 56.8\% \\
            & \texttt{skills} list absent                  &  57 & 22.2\% \\
Endpoint    & \texttt{url} missing or non-HTTPS            &  56 & 21.8\% \\
Versioning  & \texttt{version} absent                      &  14 &  5.4\% \\
\bottomrule
\end{tabular}}
\end{table}

